Zero-Shot Object Counting with Language-Vision Models

Class-agnostic object counting aims to count object instances of an arbitrary class at test time. It is challenging but also enables many potential applications. Current methods require human-annotated exemplars as inputs which are often unavailable for novel categories, especially for autonomous systems. Thus, we propose zero-shot object counting (ZSC), a new setting where only the class name is available during test time. This obviates the need for human annotators and enables automated operation. To perform ZSC, we propose finding a few object crops from the input image and use them as counting exemplars. The goal is to identify patches containing the objects of interest while also being visually representative for all instances in the image. To do this, we first construct class prototypes using large language-vision models, including CLIP and Stable Diffusion, to select the patches containing the target objects. Furthermore, we propose a ranking model that estimates the counting error of each patch to select the most suitable exemplars for counting. Experimental results on a recent class-agnostic counting dataset, FSC-147, validate the effectiveness of our method.

==> bak.tex <==
\begin{table*}[!h] 
  \centering
\resizebox{0.7\textwidth}{!}{%
  \begin{tabular}{l|c|cccc|cccc}
    \toprule
   \multirow{2}{*}{Baseline} & \multirow{2}{*}{Exemplars} & \multicolumn{4}{c|}{Val Set} & \multicolumn{4}{c}{Test Set} \\
    & & MAE & RMSE & NAE & SRE & MAE & RMSE & NAE & SRE \\
        \midrule
    \multirow{3}{*}{FamNet+} & {RPN} & {42.85} & {121.59} & 0.75 & 6.94 & {42.70} & {146.08}  & 0.74 & 7.14 \\
    & Patch-Sel (VAE) & 39.51 & 101.70 & 0.84 & 6.80 & 39.91 & {143.04} & 0.74 & 6.77 \\
    & Patch-Sel (SD) & \textbf{34.60} & \textbf{96.76} & \textbf{0.63} & \textbf{5.71} & \textbf{32.71} & \textbf{139.93}  & \textbf{0.55} & \textbf{5.47} \\
    \midrule
    \multirow{3}{*}{BMNet} & {RPN} & {37.26} & {108.54} & 0.42 & 5.43 & {37.22} & {143.13} & 0.41 & 5.31 \\
    & Patch-Sel (VAE) & 27.71 & 93.98 & 0.36 & 4.55 & 24.45 & {130.42} & 0.33 & 4.09 \\
    & Patch-Sel (SD) & \textbf{26.53} & \textbf{91.55} & \textbf{0.32} & \textbf{4.36} & \textbf{22.27} & \textbf{129.67}  & \textbf{0.28} & \textbf{3.85} \\
    \midrule
    \multirow{3}{*}{BMNet+} & {RPN} & {35.51} & {106.07} & 0.41 & 5.28 & {34.52} & {132.64} & 0.39 & 5.26 \\
    & Patch-Sel (VAE) & 26.89 & 92.37 & 0.35 & 4.56 & 23.14 & {114.40} & 0.34 & 3.95 \\
    & Patch-Sel (SD) & \textbf{25.91} & \textbf{90.62} & \textbf{0.33} & \textbf{4.40} & \textbf{19.45} & \textbf{109.82}  & \textbf{0.27} & \textbf{3.53} \\
    \midrule
     \multirow{3}{*}{CounTR} 
    & {RPN} & {39.71} & {107.47} & 0.48 & 5.91 & {47.65} & {149.73} & 0.59 & 6.75  \\
    & Patch-Sel (VAE) & {25.42} & {95.77} & \textbf{0.32} & \textbf{4.54} & \textbf{17.68} & \textbf{107.21} & \textbf{0.27} & \textbf{4.40} \\
    & Patch-Sel (SD) &  \textbf{24.41} & \textbf{92.68} & {0.34} & {5.12} & 19.55 & 113.14 & 0.30 & 7.42  \\
    \multirow{3}{*}{SAFECount} & {RPN} & {34.98} & {107.46} & 0.38 & 5.22 & {33.89} & {139.92} & 0.39 & 5.34 \\
    & Patch-Sel (VAE) & 28.34 & 94.22 & 0.41 & 4.65 & 23.60 & \textbf{110.95} & 0.40 & \textbf{4.26} \\
    & Patch-Sel (SD) & \textbf{26.85} & \textbf{91.09} & \textbf{0.33} & \textbf{4.30} & \textbf{21.44} & {115.30}  & \textbf{0.30} & 5.74 \\
    \bottomrule
  \end{tabular}} \\  \vspace{4pt}
  \caption{ Quantitative comparisons on the FSC-147 dataset. ``GT" denotes using human-annotated boxes as exemplars. ``RPN" denotes using the top-3 RPN proposals with the highest objectness scores as exemplars. ``Patch-Selection" denotes using our selected patches as exemplars.
  }\label{tab:baselines}%
  \vspace{0pt}
\end{table*}



\begin{table}[!h] 
  \centering
\resizebox{0.46\textwidth}{!}{%
  \begin{tabular}{l|c|cc|cc}
    \toprule
   \multirow{2}{*}{Baseline} & \multirow{2}{*}{Exemplars} & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    & & MAE & RMSE & MAE & RMSE  \\
        \midrule
    \multirow{3}{*}{FamNet+} & {RPN} & {42.85} & {121.59} & {42.70} & {146.08}  \\
    & Patch-Sel (VAE) & 39.51 & 101.70 & 39.91 & {143.04}  \\
    & Patch-Sel (SD) & \textbf{34.60} & \textbf{96.76} & \textbf{32.71} & \textbf{139.93} \\
    \midrule
    \multirow{3}{*}{BMNet} & {RPN} & {37.26} & {108.54} & {37.22} & {143.13} \\
    & Patch-Sel (VAE) & 27.71 & 93.98 & 24.45 & {130.42} \\
    & Patch-Sel (SD) & \textbf{26.53} & \textbf{91.55}  & \textbf{22.27} & \textbf{129.67}  \\
    \midrule
    \multirow{3}{*}{BMNet+} & {RPN} & {35.51} & {106.07} & {34.52} & {132.64} \\
    & Patch-Sel (VAE) & 26.89 & 92.37 & 23.14 & {114.40}  \\
    & Patch-Sel (SD) & \textbf{25.91} & \textbf{90.62} & \textbf{19.45} & \textbf{109.82}  \\
    \midrule
     \multirow{3}{*}{CounTR} 
    & {RPN} & {39.71} & {107.47} & {47.65} & {149.73}  \\
    & Patch-Sel (VAE) & {25.42} & {95.77}  & \textbf{17.68} & \textbf{107.21}\\
    & Patch-Sel (SD) &  \textbf{24.41} & \textbf{92.68} & 19.55 & 113.14   \\
    \midrule
    \multirow{3}{*}{SAFECount} & {RPN} & {34.98} & {107.46} & {33.89} & {139.92}  \\
    & Patch-Sel (VAE) & 28.34 & 94.22 & 23.60 & \textbf{110.95}  \\
    & Patch-Sel (SD) & \textbf{26.85} & \textbf{91.09} &  \textbf{21.44} & {115.30}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{2mm}
  \caption{ Quantitative comparisons on the FSC-147 dataset. ``GT" denotes using human-annotated boxes as exemplars. ``RPN" denotes using the top-3 RPN proposals with the highest objectness scores as exemplars. ``Patch-Selection" denotes using our selected patches as exemplars.
  }\label{tab:baselines2}%
  \vspace{5pt}
\end{table}

\begin{table}[!h] 
  \centering
\resizebox{0.48\textwidth}{!}{%
  \begin{tabular}{c|cccc|cccc}
    \toprule
   {Prototype} & \multicolumn{4}{c|}{Val Set} & \multicolumn{4}{c}{Test Set} \\
    {Patches} &  MAE & RMSE & NAE & SRE & MAE & RMSE & NAE & SRE \\
    \midrule
    %top-1 &  26.76 & \textbf{88.37} & 0.36 & 4.36 & 21.89 &  113.50 & 0.33 & 3.79 \\
    top-5  & \textbf{26.30} & \textbf{88.80} & {0.34} & \textbf{4.27} & \textbf{21.53} & \textbf{113.28} & \textbf{0.31} & {3.61} \\
    top-25  & 26.35 & 90.74 & \textbf{0.33} & 4.29 & 21.65 & 113.41 & 0.31 & \textbf{3.60} \\ 
    top-50  & 26.75 & 91.51 & 0.33 & 4.31 & 21.54 & 113.70 & 0.31 & 3.57 \\ 
    \midrule
    all  & 27.91 & 94.48 & 0.34 & 4.42 & 22.84 & 115.81 & 0.31 & 3.69 \\ 
    \bottomrule
  \end{tabular}} \\ \vspace{2mm}
  \caption{ Ablation study on each component's contribution to the final results. We show the effectiveness of the two steps of our framework: selecting class-relevant patches via a generated class prototype and selecting optimal patches via an error predictor.
  }\label{tab:patches_num} \vspace{2mm}
\end{table}


\begin{table*}[!h] 
  \centering
\resizebox{0.7\textwidth}{!}{%
  \begin{tabular}{c|c|cccc|cccc}
    \toprule
   \multirow{2}{*}{\parbox{1.5cm}{Patch \\ selection}}& \multirow{2}{*}{\parbox{2cm}{Class Prototype}} & \multicolumn{4}{c|}{Val Set} & \multicolumn{4}{c}{Test Set} \\
    & & MAE & RMSE & NAE & SRE & MAE & RMSE & NAE & SRE \\
    \midrule
    \xmark & VAE-generated & {48.55} & {127.92} & 0.65 & 6.37 & {41.33} & {147.43} & 0.52 & 5.53 \\ 
    \xmark & SD-generated & {30.51} & {101.39} & 0.41 & 4.66 & {28.03} & {132.34} & 0.37 & 4.42 \\
    %\Checkmark & MS-COCO & \textbf{27.00} & \textbf{87.90} & \textbf{0.35} & \textbf{4.29} & \textbf{22.09} & \textbf{115.17} & \textbf{0.34} & \textbf{3.74} \\
    \Checkmark & MS-COCO & \textbf{26.30} & \textbf{88.80} & \textbf{0.34} & \textbf{4.27} & \textbf{21.53} & \textbf{113.28} & \textbf{0.31} & \textbf{3.61} \\
    \bottomrule
  \end{tabular}} \\ \vspace{4pt}
  \caption{ {Comparison between our proposed method and the baseline approach of directly using the generated class prototype to do correlation matching.} 
  }\label{tab:patch_selection}%
  \vspace{-10pt}
\end{table*}
